Codes for Preventing Zeros at Partially Defective Memory Positions

This work deals with error correction for non-volatile memories that are partially defective at some levels. Such memory cells can only store incomplete information since some of their levels cannot be utilized entirely due to, e.g., wearout. On top of that, this paper corrects random errors $t\geq 1$ that could happen among $u$ partially defective cells while preserving their constraints. First, we show that the probability of violating the partially defective cells' restriction due to random errors is not trivial. Next, we update the models in [1] such that the coefficients of the output encoded vector plus the error vector at the partially defective positions are non-zero. Lastly, we state a simple proposition (Proposition 3) for masking the partial defects using a code with a minimum distance $d$ such that $d\geq 2(u+t)+1$. "Masking" means selecting a word whose entries correspond to writable levels in the (partially) defective positions. A comparison shows that masking $u$ cells by this proposition for a particular BCH code is as effective as using the complicated coding scheme proven in [1, Theorem 1].

==> Codes_for_Preventing_Zeros_at_Partially_Defect_Memory_Positions_ITW- Reviewers_arXiv/Block_diagram_A.tex <==
 \begin{tikzpicture}[auto, thick, >=triangle 45]
    \node[draw, thick, rectangle, minimum height = 2.5em, minimum width = 2.5em] at (1.4,0) (matrix) {$\boldsymbol{G}_1$};
    \node[draw, circle, minimum size=0.2cm] (adder1) at (3.3,0){};
    \draw (adder1.east) -- (adder1.west) (adder1.north) -- (adder1.south);
    \node[draw, circle, minimum size=0.2cm] (adder2) at (5.8,0){};
    \draw (adder2.east) -- (adder2.west) (adder2.north) -- (adder2.south);
    
    \coordinate (message) at (0,0);
    \coordinate (masking) at (3.3,1.4);
    \coordinate (error) at (5.8,1.4);
    \coordinate (corrupted) at (8.2,0);
    
    \draw[-latex](message) -- node {$\boldsymbol{m}$}(matrix);
    \draw[-latex](matrix) -- node {$\boldsymbol{w},w_{i}$}(adder1);
    \draw[-latex](adder1) -- node {$c_{i}\in\mathbb{F}_q\backslash\{0\}$}(adder2);
    \draw[-latex](masking) -- node {$d_{i}$}(adder1);
    \draw[-latex](error) -- node {$e_{j}\in\{0,1\}$}(adder2);
    \draw[-latex](adder2) -- node {$y_{i,j}\in\mathbb{F}_q\backslash\{0\}$}(corrupted);
    
    \draw[color=gray,thick](0.7,-0.7) rectangle (4,1.1);
	\node at (0.5,1.3) [above=5mm, right=0mm] {\textsc{encoder}};
	
	\draw[dashed] (2.4,-1) -- (2.4,1.7);
    \end{tikzpicture}

==> Codes_for_Preventing_Zeros_at_Partially_Defect_Memory_Positions_ITW- Reviewers_arXiv/Block_diagram_B.tex <==
   \begin{tikzpicture}[auto, thick, >=triangle 45]
    \node[draw, thick, rectangle, minimum height = 2.5em, minimum width = 2.5em] at (1.4,0) (matrix) {$\boldsymbol{G}_1$};
    \node[draw, circle, minimum size=0.2cm] (adder1) at (3.3,0){};
    \draw (adder1.east) -- (adder1.west) (adder1.north) -- (adder1.south);
    \node[draw, circle, minimum size=0.2cm] (adder2) at (6.8,0){};
    \draw (adder2.east) -- (adder2.west) (adder2.north) -- (adder2.south);
    
    \coordinate (message) at (0,0);
    \coordinate (masking) at (3.3,1.4);
    \coordinate (error) at (6.8,1.4);
    \coordinate (corrupted) at (9.2,0);
    
    \draw[-latex](message) -- node {$\boldsymbol{m}$}(matrix);
    \draw[-latex](matrix) -- node {$\boldsymbol{w},w_{i}$}(adder1);
    \draw[-latex](adder1) -- node {$c_{i}\in\mathbb{F}_q\backslash\{0,q-1\}$}(adder2);
    \draw[-latex](masking) -- node {$d_{i}$}(adder1);
    \draw[-latex](error) -- node {$e_{j}\in\{0,1\}$}(adder2);
    \draw[-latex](adder2) -- node {$y_{i,j}\in\mathbb{F}_q\backslash\{0\}$}(corrupted);
    
    \draw[color=gray,thick](0.7,-0.7) rectangle (4,1.1);
	\node at (0.5,1.3) [above=5mm, right=0mm] {\textsc{encoder}};
	
	\draw[dashed] (2.4,-1) -- (2.4,1.7);
    \end{tikzpicture}

==> Codes_for_Preventing_Zeros_at_Partially_Defect_Memory_Positions_ITW- Reviewers_arXiv/Half_u_graph.tex <==
\begin{tikzpicture}
\begin{axis}[
    title={},
    xlabel={Prime $q$},
    ylabel={Masking capability $u$},
    xmin=0, xmax=200,
    ymin=0, ymax=200,
    xtick={0,20,40,60,80,100,120,140,160,180,200},
    ytick={0,20,40,60,80,100,120,140,160,180,200},
    legend pos=north west,
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=dashed,
]

\addplot[color=black, mark=+,]
    coordinates {
    (2,1)(3,2)(5,4)(7,6)(11,10)(13,12)(17,16)(19,18)(23,22)(29,28)(31,30)(37,36)(41,40)(43,42)(47,46)(53,52)(59,58)(61,60)(67,66)(71,70)(73,72)(79,78)(83,82)(89,88)(97,96)(101,100)(103,102)(107,106)(109,108)(113,112)(127,126)(131,130)(137,136)(139,138)(149,148)(151,150)(157,156)(163,162)(167,166)(173,172)(179,178)(181,180)(191,190)(193,192)(197,196)(199,198)
    };
    \addlegendentry{\cite[Theorem ~1]{haideralkim2019psmc}}
    
\addplot[color=blue, mark=+,]
    coordinates {
    (3,1)(5,2)(7,3)(11,5)(13,6)(17,8)(19,9)(23,11)(29,14)(31,15)(37,18)(41,20)(43,21)(47,23)(53,26)(59,29)(61,30)(67,33)(71,35)(73,36)(79,39)(83,41)(89,44)(97,48)(101,50)(103,51)(107,53)(109,54)(113,56)(127,63)(131,65)(137,68)(139,69)(149,74)(151,75)(157,78)(163,81)(167,83)(173,86)(179,89)(181,90)(191,95)(193,96)(197,98)(199,99)
    };
    \addlegendentry{Theorem \ref{Theorem_1}}
\end{axis}
\end{tikzpicture}

==> Codes_for_Preventing_Zeros_at_Partially_Defect_Memory_Positions_ITW- Reviewers_arXiv/defs.tex <==
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepackage{tikz}
\usetikzlibrary{arrows,matrix,positioning,patterns}
\usepackage[utf8]{inputenc}
\usepackage[innermargin=0.75in,outermargin=0.75in,top=0.5in,bottom=0.6in]{geometry}
\setlength{\columnsep}{0.18 in}
\usepackage[english]{babel}
\usepackage[T1]{fontenc}
\usepackage{epsfig}
\usepackage{amsmath, amssymb, amsbsy}
\usepackage{mathdots}
\usepackage{xspace}
\usepackage[noend]{algpseudocode}
\usepackage[linesnumbered,ruled,vlined,titlenumbered]{algorithm2e}
\usepackage{algorithmicx}
\usepackage{color}
\usepackage{cite}
\usepackage{booktabs}
\usepackage{verbatim}
\usepackage{url}
\usepackage{lipsum}
\usepackage{enumitem}
\usepackage{colortbl}
\usepackage{amsthm}
\usepackage{dblfloatfix}
\usepackage{verbatim}
\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother


\usepackage{multicol}


\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{question}[theorem]{Question}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{openproblem}{Open Research Problem}
\newtheorem{definition}{Definition}

\usepackage[final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=10,shrink=20]{microtype}



\newenvironment{mymatrix}{\begin{bmatrix}} {\end{bmatrix} }


\def\ve#1{{\mathchoice{\mbox{\boldmath$\displaystyle #1$}}
              {\mbox{\boldmath$\textstyle #1$}}
              {\mbox{\boldmath$\scriptstyle #1$}}
              {\mbox{\boldmath$\scriptscriptstyle #1$}}}}

\newcommand{\todo}[1]{{\color{red}[#1]}}
\newcommand{\pu}[1]{{\color{orange}[pu: #1]}}
\newcommand{\aw}[1]{{\color{blue}[aw: #1]}}
\newcommand{\jr}[1]{{\color{blue}[jr: #1]}}


\renewcommand{\vec}[1]{\ensuremath{\boldsymbol{#1}}}

\newcommand{\Mooremat}[3]{\ensuremath{\mathcal{M}_{#1,#2}\left( #3 \right)}}
\newcommand{\MoormatExplicit}[3]{
	\begin{mymatrix}
		#1_{1} & #1_{2} & \dots& #1_{#3}\\
		#1_{1}^{[1]} & #1_{2}^{[1]} & \dots& #1_{#3}^{[1]}\\
		\vdots &\vdots&\ddots& \vdots\\
		#1_{1}^{[#2-1]} & #1_{2}^{[#2-1]} & \dots& #1_{#3}^{[#2-1]}\\
	\end{mymatrix}}

\newcommand{\MoormatExplicitMat}[4]{
	\begin{pmatrix}
          #1_{1,1} & #1_{1,2} & \dots& #1_{1,#3}\\
          #1_{2,1} & #1_{2,2} & \dots& #1_{2,#3}\\
          \vdots &\vdots&\ddots& \vdots\\
          #1_{#4,1} & #1_{#4,2} & \dots& #1_{#4,#3}\\
          #1_{1,1}^{q} & #1_{1,2}^{q} & \dots& #1_{1,#3}^{q}\\
          #1_{2,1}^{q} & #1_{2,2}^{q} & \dots& #1_{2,#3}^{q}\\
                    \vdots &\vdots&\ddots& \vdots\\
		#1_{#4,1}^{q^{#2-1}} & #1_{#4,2}^{q^{#2-1}} & \dots& #1_{#4,#3}^{q^{#2-1}}\\
	\end{pmatrix}}


      
\newcommand{\Fq}{\ensuremath{\mathbb{F}_q}}
\newcommand{\Fqm}{\ensuremath{\mathbb{F}_{q^m}}}
\newcommand{\Fqml}{\ensuremath{\mathbb{F}_{q^{m\ell}}}}
\newcommand{\Fqmu}{\ensuremath{\mathbb{F}_{q^{mu}}}}
\newcommand{\Lfield}{\ensuremath{\mathbb{L}}}

\DeclareMathOperator{\extsmallfield}{ext}
\DeclareMathOperator{\rank}{rk}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\LambdaOp}{\Lambda}
\newcommand{\Code}{\mathcal{C}}
\newcommand{\IC}{\mathcal{IC}}
\newcommand{\qpow}[1]{^{[#1]}}
\newcommand{\rspace}[2]{\mathcal{R}_{#2} \begin{pmatrix}#1\end{pmatrix}}
\newcommand{\nkhalffrac}{\left\lfloor \frac{n-k}{2}\right\rfloor}


\newcommand{\rref}[1]{\text{ref}(#1) }
\renewcommand{\ker}{\mathcal{K} }

\newcommand{\RkExbrror}{\ensuremath{\varphi}}
\newcommand{\dimZ}{\ensuremath{\zeta}}
\newcommand{\MooreZ}{\ensuremath{\tilde{\ve{Z}}}}


\newcommand{\tpub}{\ensuremath{t_{\mathsf{pub}}}}
\newcommand{\kpub}{\ensuremath{\mathbf{k}_{\mathsf{pub}}}}
\newcommand{\mycode}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\fontmetric}[1]{\mathsf{#1}}
\newcommand{\codeRank}[1]{\ensuremath{(#1)_q^\fontmetric{R}}}
\newcommand{\codelinearRank}[1]{\ensuremath{[#1]_q^\fontmetric{R}}}

\newcommand{\Gabcode}[2]{\ensuremath{\mathcal{G}(#1,#2)}}
\newcommand{\IntGabcode}[1]{\ensuremath{\mathcal{IG}(#1)}}
\newcommand{\IntCode}[1]{\ensuremath{\mathcal{IC}[#1]}}


\newcommand{\numbRowErasures}{\varrho}
\newcommand{\numbColErasures}{\gamma}

\newcommand{\0}{\ve{0}}
\renewcommand{\S}{\ve{S}}
\renewcommand{\H}{\ve{H}}
\newcommand{\y}{\ve{y}}
\renewcommand{\a}{\ve{a}}
\renewcommand{\b}{\ve{b}}
\newcommand{\e}{\ve{e}}
\renewcommand{\v}{\ve{v}}
\newcommand{\g}{\ve{g}}
\newcommand{\m}{\ve{m}}
\renewcommand{\c}{\ve{c}}
\renewcommand{\e}{\ve{e}}
\renewcommand{\m}{\ve{m}}
\newcommand{\G}{\ve{G}}
\renewcommand{\P}{\ve{P}}
\newcommand{\R}{\ve{R}}
\newcommand{\K}{\ve{K}}
\newcommand{\M}{\ve{M}}
\newcommand{\E}{\ve{E}}
\newcommand{\C}{\ve{C}}
\newcommand{\Y}{\ve{Y}}
\newcommand{\HE}{\ve{H}_{\text{E}}}
\newcommand{\Gpub}{\ve{G}_\mathrm{pub}}
\newcommand{\Hpub}{\ve{H}_\mathrm{pub}}
\newcommand{\Hsub}{\ve{H}_\mathrm{sub}}
\newcommand{\Hsubi}{\ve{H}_{\mathrm{sub},i}}
\newcommand{\HsubEins}{\ve{H}_{\mathrm{sub},1}}
\newcommand{\HsubNKT}{\ve{H}_{\mathrm{sub},n-k-t}}
\newcommand{\new}[1]{{\color{blue} #1}}
\newcommand{\A}{\ve{A}}
\newcommand{\B}{\ve{B}}
\newcommand{\Bp}{\ve{B}^{\prime }}
\newcommand{\Bppt}{\ve{B}^{\prime \prime \top}}
\newcommand{\Bpp}{\ve{B}^{\prime \prime}}
\newcommand{\Hp}{\ve{H}^{\prime}}
\newcommand{\hp}{\ve{h}^{\prime}}
\newcommand{\h}{\ve{h}}
\newcommand{\Htil}{\tilde{\ve{\H}}}
\newcommand{\I}{\ve{I}}
\newcommand{\J}{\ve{J}}
\newcommand{\D}{\ve{D}}
\newcommand{\Dp}{\ve{D}^{\prime}}


\newcommand{\dE}{d_\mathrm{E}}
\renewcommand{\AE}{\A_\mathrm{E}}
\newcommand{\BE}{\B_\mathrm{E}}
\newcommand{\dR}{\mathrm{d}_\mathrm{R}}
\newcommand{\dH}{\mathrm{d}_\mathrm{H}}
\newcommand{\Matmap}{\varphi}

\newcommand{\wtR}{\mathrm{wt}_\mathrm{R}}

\newcommand{\Binv}{\B_\mathrm{inv}}
\newcommand{\Bker}{\B_\mathrm{ker}}
\newcommand{\GaugY}{\G_\mathrm{aug}^{\cipher}}
\newcommand{\GaugE}{\G_\mathrm{aug}^{\E}}
\newcommand{\CodeE}{\Code_\E}
\newcommand{\Caug}{\Code_\mathrm{aug}}
\newcommand{\Ctwisted}{\Code_\mathrm{twisted}}

\newcommand{\NMtnm}{\mathrm{NM}_{t,n,m}}
\newcommand{\CGab}{\Code_\mathcal{G}}

\newcommand{\tauSB}{\tau_\mathrm{SB}}
\newcommand{\boundSB}{\varrho_\mathrm{SB}}
\newcommand{\CSB}{C_\mathrm{SB}}
\newcommand{\tauLO}{\tau_\mathrm{LO}}
\newcommand{\boundLO}{\varrho_\mathrm{LO}}
\newcommand{\CLO}{C_\mathrm{LO}}
\newcommand{\tauWZ}{\tau_\mathrm{WZ}}
\newcommand{\boundWZ}{\varrho_\mathrm{WZ}}
\newcommand{\CWZ}{C_\mathrm{WZ}}

\newcommand{\suppR}{\mathrm{supp}_\mathrm{R}}
\newcommand{\suppH}{\mathrm{supp}_\mathrm{H}}
\newcommand{\ranksupp}[1]{\suppR(#1)}


\newcommand{\Fqmell}{\mathbb{F}_{q^{m \ell}}}

\newcommand{\tmax}{t_\mathrm{max}}
\newcommand{\Z}{\ve{Z}}
\newcommand{\F}{\mathbb{F}}



==> Half_u_graph.tex <==
\begin{tikzpicture}
\begin{axis}[
    title={},
    xlabel={Prime $q$},
    ylabel={Masking capability $u$},
    xmin=0, xmax=200,
    ymin=0, ymax=200,
    xtick={0,20,40,60,80,100,120,140,160,180,200},
    ytick={0,20,40,60,80,100,120,140,160,180,200},
    legend pos=north west,
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=dashed,
]

\addplot[color=black, mark=+,]
    coordinates {
    (2,1)(3,2)(5,4)(7,6)(11,10)(13,12)(17,16)(19,18)(23,22)(29,28)(31,30)(37,36)(41,40)(43,42)(47,46)(53,52)(59,58)(61,60)(67,66)(71,70)(73,72)(79,78)(83,82)(89,88)(97,96)(101,100)(103,102)(107,106)(109,108)(113,112)(127,126)(131,130)(137,136)(139,138)(149,148)(151,150)(157,156)(163,162)(167,166)(173,172)(179,178)(181,180)(191,190)(193,192)(197,196)(199,198)
    };
    \addlegendentry{\cite[Theorem ~1]{haideralkim2019psmc}}
    
\addplot[color=blue, mark=+,]
    coordinates {
    (3,1)(5,2)(7,3)(11,5)(13,6)(17,8)(19,9)(23,11)(29,14)(31,15)(37,18)(41,20)(43,21)(47,23)(53,26)(59,29)(61,30)(67,33)(71,35)(73,36)(79,39)(83,41)(89,44)(97,48)(101,50)(103,51)(107,53)(109,54)(113,56)(127,63)(131,65)(137,68)(139,69)(149,74)(151,75)(157,78)(163,81)(167,83)(173,86)(179,89)(181,90)(191,95)(193,96)(197,98)(199,99)
    };
    \addlegendentry{Theorem \ref{Theorem_1}}
\end{axis}
\end{tikzpicture}
